Experience Report: Towards Moving Things with Types -- Helping Logistics Domain Experts to Control Cyber-Physical Systems with Type-Based Synthesis

One of the ultimate goals of software engineering is to leave virtual spaces and move real things. We take one step toward supporting users with this goal by connecting a type-based synthesis algorithm, (CL)S, and its IDE to a logistics lab environment. The environment is built and used by domain experts, who have little or no training in formal methods, and need to cope with large spaces of software, hardware and problem specific solution variability. It consists of a number of Cyber-Physical Systems (CPS), including wheel-driven robots as well as flying drones, and it has laser-based support to visualize their possible movements. Our work describes results on an experiment integrating the latter with (CL)S. Possibilities and challenges of working in the domain of logistics and in cooperation with its experts are outlined. Future research plans are presented and an invitation is made to join the effort of building better, formally understood, development tools for CPS-enabled industrial environments.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{R. Monahan, V. Prevosto, J. Proen\c{c}a (Eds.): Formal\\
Integrated Development Environment 2019 (F-IDE 2019)\\
EPTCS 310, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.310.1}{10.4204/EPTCS.310.1}}
\pdfoutput=1

